OpenIllumination: A Multi-Illumination Dataset for Inverse Rendering Evaluation on Real Objects

We introduce OpenIllumination, a real-world dataset containing over 108K images of 64 objects with diverse materials, captured under 72 camera views and a large number of different illuminations. For each image in the dataset, we provide accurate camera parameters, illumination ground truth, and foreground segmentation masks. Our dataset enables the quantitative evaluation of most inverse rendering and material decomposition methods for real objects. We examine several state-of-the-art inverse rendering methods on our dataset and compare their performances. The dataset and code can be found on the project page: https://oppo-us-research.github.io/OpenIllumination.

==> figures/greenhead.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/greenhead1_CA2.JPG}
    \caption{\textbf{The light stage we used to capture the images.}
    The light stage contains 48 DSLR Canon cameras and 142 LED lights.
    }
    \label{fig:lightstage}
\end{figure}

==> figures/stats.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/stats_v2.pdf}
%    \vspace{-1em}
    \caption{Material distribution in the proposed dataset.  The labels are from OpenSurfaces~\cite{bell2013opensurfaces}.}\label{fig:stats}
    % \vspace{-4em}
    \label{fig:stats}
\end{figure}

==> figures/stats_greenhead_mirrorball.tex <==
\begin{figure}[!htb]
\CenterFloatBoxes
\RawFloats
\begin{floatrow}
\minipage{0.32\textwidth}
% \vspace{11pt}
  \includegraphics[width=\linewidth]{figures/material_list2.pdf}
  \centering
  \caption{Material distribution in the proposed dataset.  The labels are from OpenSurfaces~\cite{bell2013opensurfaces}.}\label{fig:stats}
\endminipage\hfill
\hspace{3pt}
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/NC3.jpg}
  \centering
    \caption{An example image of a green head used for camera calibration.}%
  \label{fig:greenhead}
\endminipage\hfill
\hspace{3pt}
\minipage{0.32\textwidth}%
\vspace{11pt}
  \includegraphics[width=\linewidth]{figures/mirrorballv2.jpg}
  \centering
    \caption{An example image of the chrome ball. We captured OLAT images for the mirror ball for lighting calibration.} 
  \label{tab:mirrorball}
\endminipage
\end{floatrow}
\end{figure}
